Moniqua: Modulo Quantized Communication in Decentralized SGD

Running Stochastic Gradient Descent (SGD) in a decentralized fashion has shown promising results. In this paper we propose Moniqua, a technique that allows decentralized SGD to use quantized communication. We prove in theory that Moniqua communicates a provably bounded number of bits per iteration, while converging at the same asymptotic rate as the original algorithm does with full-precision communication. Moniqua improves upon prior works in that it (1) requires zero additional memory, (2) works with 1-bit quantization, and (3) is applicable to a variety of decentralized algorithms. We demonstrate empirically that Moniqua converges faster with respect to wall clock time than other quantized decentralized algorithms. We also show that Moniqua is robust to very low bit-budgets, allowing 1-bit-per-parameter communication without compromising validation accuracy when training ResNet20 and ResNet110 on CIFAR10.

==> section/convergence_analysis.tex <==
\section{Convergence Analysis}
We make the following assumptions here:
\begin{enumerate}
	\item \textbf{Lipschitzian Gradient}: All the function $f_i$ have $L_i$-Lipschitzian gradients.\label{Assumption1}
	\begin{displaymath}
	\left\|\nabla f_i(x) - \nabla f_i(y)\right\|\leq L_i\left\|x-y\right\|, \forall i\in [n]
	\end{displaymath}
	And define $L=\max_i\{L_i\}$.
	\item \textbf{Spectral Gap}: Communication matrix $W$ is a symmetric doubly stochastic matrix and for $\rho\triangleq\max\{|\lambda_2(W)|, |\lambda_n(W)|\}$, $\rho<1$.\label{Assumption2}
	\item \textbf{Bounded Variance}:
		%\begin{displaymath}
			\begin{align*}
			& \mathbb{E}_{\xi_i\sim\mathcal{D}_i}\left\|\nabla\widetilde{f}_i(x;\xi_i) - \nabla f_i(x)\right\|^2 \leq \sigma^2, \forall i\\
			& \mathbb{E}_{i\sim\mathcal{U}([n])}\left\|\nabla f_i(x) - \nabla f(x)\right\|^2 \leq \varsigma^2, \forall i\\
			\end{align*}
		%\end{displaymath}
		For one worker, the first inequality shows that inter variance is bounded by some constant $\sigma^2$. The second inequality shows intra variance is bounded by some constant $\varsigma^2$. \label{Assumption3}
	\item \textbf{Initialization}: All the workers start from the same point, and without the loss of generality, we have $x_{0,i}=0, \forall i$ \label{Assumption4}
	\item \textbf{Bounded sample gradient norm}: For any subgradient $\widetilde{g}_{k,i}$ sampled by $i$ at iteration $k$, we have$\left\|\widetilde{g}_{k,i}\right\|\leq G, \forall i$ \label{Assumption4}
\end{enumerate}
\begin{theorem}\label{QD-PSGD rate}
If we apply a general quantizer $\mathcal{Q}$ (can be biased, non-linear) such that $\left\|\mathcal{Q}(z)-z\right\|^2\leq\omega^2\left\|z\right\|^2, \forall z\in\mathbb{R}^d$, where $\omega$ is a hyper parameter associated with the quantizer, make the exchanged information
\begin{displaymath}
q_{k,i}=\theta\mathcal{Q}\left(\frac{x_{k,i}}{\theta}\mod 1\right)
\end{displaymath}
And by setting $\theta=\frac{16\log(4n)\alpha G}{1-\rho}$, $\omega=\frac{1-\rho}{32\log(4n)}$ and $\alpha=\frac{1}{\varsigma^{\frac{2}{3}}K^{\frac{1}{3}}+\sigma\sqrt{\frac{K}{n}}}$, the output of Quantized D-PSGD has
\begin{equation}
%\begin{align*}
	\frac{1}{K}\sum_{k=0}^{K-1}\mathbb{E}\left\|\nabla f(\overline{X}_k)\right\|^2\lesssim \frac{\sigma}{\sqrt{nK}} + \frac{\varsigma^{\frac{2}{3}}}{K^{\frac{2}{3}}} + \frac{n}{K} + \frac{nG^2}{\sigma^2K}
%\end{align*}
\end{equation}
\end{theorem}
\paragraph{Remark 1} Note that comparing the asymptotic rate in Theorem~\ref{QD-PSGD rate} with D-PSGD \cite{lian2017can}, the quantization noise introduces $\frac{nG^2}{\sigma^2K}$, which is dominated by $\frac{\sigma}{\sqrt{nK}}$ when $K$ is sufficient large. And 
\begin{corollary}
If we use a linear quantizer with quantization length $\delta$, the number of bits required per dimension per iteration is
\begin{displaymath}
    \log\left(\frac{32\log(4n)\sqrt{d}}{1-\rho}\right)
\end{displaymath}
\end{corollary}
